Data-Efficient Prediction of Minimum Operating Voltage via Inter- and Intra-Wafer Variation Alignment

Predicting the minimum operating voltage ($V_{min}$) of chips stands as a crucial technique in enhancing the speed and reliability of manufacturing testing flow. However, existing $V_{min}$ prediction methods often overlook various sources of variations in both training and deployment phases. Notably, the neglect of wafer zone-to-zone (intra-wafer) variations and wafer-to-wafer (inter-wafer) variations, compounded by process variations, diminishes the accuracy, data efficiency, and reliability of $V_{min}$ predictors. To address this gap, we introduce a novel data-efficient $V_{min}$ prediction flow, termed restricted bias alignment (RBA), which incorporates a novel variation alignment technique. Our approach concurrently estimates inter- and intra-wafer variations. Furthermore, we propose utilizing class probe data to model inter-wafer variations for the first time. We empirically demonstrate RBA's effectiveness and data efficiency on an industrial 16nm automotive chip dataset.

==> tex/alg_rba.tex <==
\begin{algorithm} 
\caption{Restricted Bias Alignment (RBA) for $\Vmin$ Prediction}
\begin{algorithmic}[1]

\State \textbf{Input:} Training data $\{ (\X_{i,j}, \Y_{i,j} \}$ ($i=1,\cdots,N$, $j=1,\cdots,M$), class probe data $\{\z_i\}_{i=1}^N$, learning rate $\eta$, stop criterion $\tau$. 

\State \textbf{Output:} Parametric feature weight $\widehat{\w}$, class probe feature weight $\widehat{\w}_{\z}$, inter-wafer voltage biases $\{\widehat{\bias}^{inter}_i\}_{i=1}^N$, intra-wafer voltage biases $\{\widehat{\bias}^{inter}_j\}_{j=1}^M$, class probe feature bias $\widehat{\bias}_{\z}$

\State Initialize $\widehat{\w}$, $\{\widehat{\bias}^{inter}_i\}_{i=1}^N$, and $\{\widehat{\bias}^{inter}_j\}_{j=1}^M$ via \cref{eq:ba-w} and \cref{eq:ba-bias}

\State $\bm{FOM}_{init} \gets \text{Simulate the circuit with parameters } \bm{x}_{init}$
\State Fit an initial surrogate model $\gp$ on $(\bm{x}_{init}, \bm{FOM}_{init})$

\While{True}
    \State Select the next point for simulation via maximizing the acquisition function $\alpha$: $x_t \gets \arg \max_{x} \alpha(x, \gp)$
    \State $FOM_t \gets \text{Simulate the circuit with parameters } x_t$
    \State \text{Update the surrogate model $\gp$ with $(x_t, FOM_t)$}
\EndWhile

\end{algorithmic}\label{alg:bo}
\end{algorithm}
